SAE Interprets MoE: Sparse AutoEncoders Reveal That MoE Experts Exhibit Human-Interpretable Fine-Grained Specialization

Mixture-of-Experts (MoE) models route each token to a few of many experts, yet what an individual expert is responsible for remains unsettled. Prior analyses count how often each expert is selected on domain-labeled corpora. However, such labels impose a coarse taxonomy in advance, and selection frequency ignores how much an expert actually contributes. We instead introduce a general framework for analyzing specialization in feature space by training a sparse autoencoder (SAE) on the output of any MoE layer. Because this output is a router-weighted sum of expert outputs and the SAE encoder is affine, each latent's pre-activation decomposes into exact per-expert contributions. Aggregating these contributions over a corpus gives each expert a dominant set of latents that it primarily drives. Applying this framework to layers 4, 30 and 46 of Qwen3-30B-A3B, we find that expert contributions are far more concentrated than gating weights, and most latents are dominated by only one or two experts. Across experts, dominant sets are largely disjoint. Auto-interpreting these sets reveals a hierarchical division of labor. At a coarse level, experts cluster into domains of very unequal sizes, led by code, mathematics and text formatting. Within each domain, individual experts specialize in distinct subfields, such as Java versus front-end web code, or geometry versus arithmetic and polynomials. Finally, substantial feature overlap occurs almost exclusively between neighboring subfields of the same domain. Our project page is at https://bytedance-seed.github.io/SAE-interprets-MoE/, where we provide open-source code and links to the SAE models.

==> discussion.tex <==

\section{Discussion}
\label{app:discussion}

This appendix reports ablations that examine the validity of several assumptions made in the
main text. Each subsection states one assumption, describes a control built to test it, and
reports what the control shows.

\subsection{Contribution is concentrated beyond the magnitudes of the expert outputs}
\label{app:rotated-baseline}

\Cref{subsec:gating-vs-contribution} compares the rank profile of the contribution with that of
the gating weights, which rules out that the concentration of $C$ merely inherits the unevenness
of the router. The contribution of \Cref{eq:contribution} also scales with the norm of $u_j(t)$,
however, and the outputs of the activated experts on one prefix can differ widely in norm.
Projected onto almost any direction, the sum in \Cref{eq:decomposition} is then dominated by the
few experts whose $g_j(t)\, u_j(t)$ is largest, whether or not that direction corresponds to a
feature of the model. The gating profile does not control for this, so we compare the trained
SAE with an encoder whose directions carry no learned structure.

We draw a Haar-random orthogonal matrix $Q \in \mathbb{R}^{d \times d}$ and replace
$W_{\mathrm{enc}}$ by $W_{\mathrm{enc}} Q$. The bias $b_{\mathrm{enc}}$, the TopK selection with
$\kappa = 100$, the expert outputs $u_j(t)$ and the gating weights $g_j(t)$ are kept unchanged,
and $C$ is computed exactly as in \Cref{subsec:fraction}. Equivalently, the original SAE reads
the rotated layer output $Q\, y(t)$. The rotation preserves the norm of every encoder row and the
angle between any two rows, so the rotated encoder has the same geometry as the trained one, and
it removes only the alignment of the latents with the directions the model uses. Its latents
still activate on every prefix, since TopK always selects $\kappa$ of them, but they no longer
correspond to features. Whatever concentration the rotated encoder shows is therefore produced
by the expert outputs and the gating alone.

Encoding with $2^{20}$ latents is expensive, so both encoders are evaluated on the same
subsample of the validation set. We take $60$ shards spaced evenly over the sorted shard list,
which keeps the proportions of the three data sources, and the first $10^5$ tokens of each. This
gives $6$M tokens and about $6 \times 10^8$ (prefix, activated latent) pairs per layer. On this
subsample the profile of the trained encoder differs from the one computed on the full
validation set (\Cref{fig:rank-profile}) by at most $0.003$ at every rank, so the subsample is
representative.

% #1 层号  #2 gating  #3 contribution  #4 rotated encoder  #5 axis 选项
\newcommand{\rankprofilerotated}[5]{%
  \begin{tikzpicture}
    \begin{axis}[
      width = 0.38\textwidth, height = 0.3\textwidth,
      title = {Layer #1},
      xlabel = {rank $r$},
      xmin = -0.3, xmax = 7.3,
      ymin = 0,    ymax = 0.68,
      xtick = {0,1,2,3,4,5,6,7},
      grid = major, grid style = {gray!20},
      tick align = outside,
      legend to name = rankprofilerotatedlegend,
      legend columns = -1,
      legend cell align = left,
      legend style = {
        draw = none,
        /tikz/every even column/.append style = {column sep = 2em},
      },
      #5
    ]
      \addplot[thick, mark = *, color = black!65] coordinates {#2};
      \addlegendentry{gating $\bar g_r$}
      \addplot[thick, dashed, mark = square*, color = red!70!black] coordinates {#3};
      \addlegendentry{contribution $\bar{C}_r$, trained encoder}
      \addplot[thick, dotted, mark = triangle*, color = blue!60!black] coordinates {#4};
      \addlegendentry{contribution $\bar{C}_r$, rotated encoder}
    \end{axis}
  \end{tikzpicture}%
}

\begin{figure}[t]
  \centering
  \rankprofilerotated{4}{
    (0,0.228385) (1,0.170646) (2,0.139857) (3,0.117821)
    (4,0.101261) (5,0.088947) (6,0.079887) (7,0.073193)
  }{
    (0,0.567694) (1,0.193636) (2,0.109129) (3,0.065290)
    (4,0.037442) (5,0.018584) (6,0.006854) (7,0.001371)
  }{
    (0,0.4673) (1,0.2191) (2,0.1294) (3,0.0822)
    (4,0.0526) (5,0.0311) (6,0.0145) (7,0.0038)
  }{ylabel = {mean share}}\hfill
  \rankprofilerotated{30}{
    (0,0.230709) (1,0.169310) (2,0.137491) (3,0.116342)
    (4,0.101124) (5,0.089777) (6,0.081058) (7,0.074186)
  }{
    (0,0.512017) (1,0.185317) (2,0.115389) (3,0.078591)
    (4,0.053420) (5,0.033443) (6,0.016858) (7,0.004964)
  }{
    (0,0.4509) (1,0.2114) (2,0.1312) (3,0.0885)
    (4,0.0596) (5,0.0366) (6,0.0174) (7,0.0045)
  }{yticklabels = {}}\hfill
  \rankprofilerotated{46}{
    (0,0.221303) (1,0.167379) (2,0.140202) (3,0.119784)
    (4,0.104272) (5,0.091635) (6,0.081666) (7,0.073756)
  }{
    (0,0.626773) (1,0.158527) (2,0.089251) (3,0.056370)
    (4,0.035613) (5,0.020709) (6,0.009856) (7,0.002901)
  }{
    (0,0.4911) (1,0.2160) (2,0.1216) (3,0.0760)
    (4,0.0484) (5,0.0288) (6,0.0140) (7,0.0040)
  }{yticklabels = {}}

  \vspace{0.6em}
  \ref{rankprofilerotatedlegend}

  \caption{Rank profiles of \Cref{fig:rank-profile} together with the contribution under a
  randomly rotated copy of the encoder. The gating and trained-encoder profiles are those of the
  full validation set, and the rotated-encoder profile is computed on a subsample of $6$M tokens
  per layer.}
  \label{fig:rank-profile-rotated}
\end{figure}

\Cref{fig:rank-profile-rotated} adds the rotated encoder to the profiles of
\Cref{fig:rank-profile}. The rotated profile is already far steeper than the gating profile, with
$\bar{C}_0 = 0.467$, $0.451$ and $0.491$ at layers 4, 30 and 46 against $\bar{g}_0 = 0.229$,
$0.231$ and $0.222$. Of the gap between $\bar{g}_0$ and the $\bar{C}_0$ of the trained encoder,
the rotated encoder thus accounts for $70\%$, $78\%$ and $66\%$. This concentration does not come
from the ReLU in \Cref{eq:contribution}, since under the rotated encoder more than $6.6$ of the
eight activated experts contribute positively to an activated latent on average. It comes from
the unevenness of $g_j(t)\, u_j(t)$ across the activated experts. The trained encoder is more
concentrated than the rotated one at every layer, reaching $\bar{C}_0 = 0.569$, $0.514$ and
$0.629$. The margins of $0.102$, $0.063$ and $0.138$ are the part of the concentration that the
magnitudes of the expert outputs do not explain.

The rank profile aggregates shares and not identities, so by itself it cannot tell whether the
expert that receives the largest share of a latent is chosen by the latent or by magnitude. We
therefore record, for every (prefix, activated latent) pair, the gating rank of its principal
contributor, the activated expert with the largest $C(j,i,x_{1:t})$. \Cref{tab:winner-rank}
reports the result. Under the rotated encoder the principal contributor is the most heavily gated
expert in $53.0\%$ to $63.4\%$ of the pairs, as expected when the projection follows magnitude.
Under the trained encoder this share falls to between $43.0\%$ and $54.8\%$. At the same time the
share of pairs won by an expert in the lower half of the gating ranking ($r \ge 4$) grows from
between $3.3\%$ and $4.0\%$ to between $7.6\%$ and $10.0\%$, a factor of $2.2$ to $2.9$.

\begin{table}[t]
  \centering
  \small
  \begin{tabular}{lcccccc}
    \hline
    & \multicolumn{2}{c}{Layer 4} & \multicolumn{2}{c}{Layer 30} & \multicolumn{2}{c}{Layer 46} \\
    Gating rank of the principal contributor & rotated & trained & rotated & trained & rotated & trained \\
    \hline
    $r = 0$ (largest $g_j$) & $61.7\%$ & $49.2\%$ & $63.4\%$ & $54.8\%$ & $53.0\%$ & $43.0\%$ \\
    $r \ge 4$               & $3.3\%$  & $9.3\%$  & $3.5\%$  & $7.6\%$  & $4.0\%$  & $10.0\%$ \\
    \hline
  \end{tabular}

  \caption{Share of (prefix, activated latent) pairs whose principal contributor sits at the given
  gating rank, under a randomly rotated copy of the encoder and under the trained encoder. Both
  are computed on the same subsample of $6$M tokens per layer.}
  \label{tab:winner-rank}
\end{table}

Most of the concentration in \Cref{fig:rank-profile} is therefore a property of the expert
outputs rather than of the latents. Which expert receives the largest share, however, depends on
the direction of the latent. The principal contributor to a trained latent is more often an
expert other than the one the router weights most heavily, and more often one from the lower half
of the gating ranking, than magnitude alone would produce. This dependence of the principal
contributor on the latent is what the main text refers to as a preference of experts over
latents.

\subsection{Dominance is not produced by routing frequency}
\label{app:routing-null}

The contribution fraction of \Cref{eq:contribution-fraction} averages $C(j,i,x_{1:t})$ over the
whole dataset, and $C(j,i,x_{1:t})$ vanishes whenever $j \notin \mathcal{A}(t)$. The value of
$s(j,i)$ therefore depends on how often $j$ is routed to on the prefixes where $i$ fires, and not
only on how much $j$ contributes there. If a latent fires mostly on one kind of token and the
router sends that kind of token to one expert, that expert could dominate the latent while
contributing no more than an average share on each prefix. In that case the dominance graph
would record selection, which is exactly the quantity \Cref{sec:intro} argues against. We test
this with two controls, both accumulated over the full validation set.

The first control keeps the routing and the concentration of every (prefix, activated latent)
pair intact and removes only the identity of the expert that receives each share. On every pair,
the $k$ values of $C(\cdot,i,x_{1:t})$ are permuted uniformly at random among the $k$ activated
experts before \Cref{eq:expected-fraction} is taken. The outcome of this control can be derived
in closed form. Given $j \in \mathcal{A}(t)$ and $i \in \mathcal{F}(t)$, expert $j$ then receives
a uniformly chosen one of $k$ values that sum to one, whose expectation is $1/k$. Since
$\sum_{j} C(j,i,x_{1:t}) = 1$ on every pair, the normalization in \Cref{eq:contribution-fraction}
divides by $\Pr[i \in \mathcal{F}(t)]$, and the permuted contribution fraction is
\begin{equation}
  \label{eq:permuted-fraction}
  s_{\mathrm{perm}}(j,i) = \frac{1}{k}\, \Pr\bigl[\, j \in \mathcal{A}(t) \bigm| i \in \mathcal{F}(t) \,\bigr] \le \frac{1}{k}.
\end{equation}
Routing frequency alone can thus give an expert at most $1/k = 0.125$ of a latent, below
$\tau = 0.2$. The same argument applied to the unpermuted fraction gives
$s(j,i) \le \mathbb{E}\bigl[C(j,i,x_{1:t}) \bigm| j \in \mathcal{A}(t),\, i \in \mathcal{F}(t)\bigr]$,
so every edge of the dominance graph belongs to an expert whose average share of the latent,
on the prefixes where both are active, exceeds $0.2$, which is $60\%$ above the $1/k$ that an
expert without preference receives. This also sharpens the reading of the threshold in
\Cref{sec:dominance_graph meta}. Besides exceeding $1/N$, $\tau$ exceeds $1/k$, the largest
fraction that routing alone can produce. The permutation run confirms the bound empirically
(\Cref{tab:routing-null}). The mean largest fraction of a latent is between $0.104$ and $0.108$,
and no latent has a dominator at $\tau = 0.2$ in any layer, whereas under the observed
contributions between $86.4\%$ and $96.3\%$ of the latents have at least one.

The permutation also separates the consistency of the principal contributor from routing. For
each latent we take the expert that is most often its principal contributor across the prefixes
on which it fires, and record the fraction of those prefixes on which that expert is the principal
contributor. Averaged over latents this fraction is $0.583$, $0.558$ and $0.608$ at layers 4, 30
and 46. After the permutation it falls to between $0.105$ and $0.109$, which is what the most
frequently co-routed expert obtains by chance. A latent is therefore won by the same expert on
more than half of the prefixes on which it fires.

The second control replaces $C(j,i,x_{1:t})$ by the gating weight $g_j(t)$, accumulated only over
the prefixes on which latent $i$ is activated. The resulting fraction is the router weight that
an expert places on the tokens where a latent fires, a selection statistic conditioned on the
latent that contains no information about contribution. Thresholded at the same $\tau = 0.2$, it
gives a dominator to $18.9\%$, $23.5\%$ and $43.1\%$ of the latents, and its edges cover only
$14.0\%$, $21.4\%$ and $31.2\%$ of the edges of the dominance graph. Where the gating graph does
have an edge, the dominance graph almost always has it too ($91.0\%$ to $97.6\%$ of the gating
edges), so the dominance graph contains the selection structure and adds a much larger part
that selection does not show.

\begin{table}[t]
  \centering
  \small
  \begin{tabular}{llccc}
    \hline
    & Statistic & Layer 4 & Layer 30 & Layer 46 \\
    \hline
    Latents with a dominator
      & contribution          & $93.0\%$ & $86.4\%$ & $96.3\%$ \\
      & gating weight         & $18.9\%$ & $23.5\%$ & $43.1\%$ \\
      & permuted contribution & $0.0\%$  & $0.0\%$  & $0.0\%$  \\
    \hline
    Mean of $\max_j s(j,i)$
      & contribution          & $0.366$ & $0.330$ & $0.423$ \\
      & gating weight         & $0.167$ & $0.168$ & $0.206$ \\
      & permuted contribution & $0.106$ & $0.104$ & $0.108$ \\
    \hline
    Winner consistency
      & contribution          & $0.583$ & $0.558$ & $0.608$ \\
      & permuted contribution & $0.107$ & $0.105$ & $0.109$ \\
    \hline
    \multicolumn{2}{l}{Dominance edges also in the gating graph} & $14.0\%$ & $21.4\%$ & $31.2\%$ \\
    \hline
  \end{tabular}

  \caption{Dominance under the observed contributions, under the gating weights accumulated on
  the prefixes where a latent fires, and under contributions permuted among the activated experts
  of each (prefix, activated latent) pair, at $\tau = 0.2$ on the full validation set. Winner
  consistency is the fraction of a latent's activated prefixes on which its most frequent
  principal contributor is the principal contributor, averaged over latents.}
  \label{tab:routing-null}
\end{table}

Two further checks concern the robustness of the dominance graph itself. A latent that fires on
only a few prefixes could have a single dominator by chance, so we group the latents by the
number of prefixes on which they activate. Fewer than $300$ latents activate on fewer than $100$
prefixes in any layer, and in every group with at least $100$ activations the share of latents
with exactly one dominator lies between $46.3\%$ and $78.3\%$, the highest value in each layer
coming from the most frequently activated latents. Single dominators are therefore not an
artifact of sparse statistics. The threshold is not critical either. At $\tau = 0.3$, $63.0\%$,
$50.4\%$ and $76.2\%$ of the latents still have a dominator, and $59.9\%$, $49.4\%$ and $69.4\%$
have exactly one.

These controls concern which experts dominate a latent and say nothing about how the dominant
sets of different experts overlap, since the permuted graph has no edges to compare.

